An analysis of full-size Russian complexly NER labelled corpus of Internet user reviews on the drugs based on deep learning and language neural nets

We present the full-size Russian complexly NER-labeled corpus of Internet user reviews, along with an evaluation of accuracy levels reached on this corpus by a set of advanced deep learning neural networks to extract the pharmacologically meaningful entities from Russian texts. The corpus annotation includes mentions of the following entities: Medication (33005 mentions), Adverse Drug Reaction (1778), Disease (17403), and Note (4490). Two of them - Medication and Disease - comprise a set of attributes. A part of the corpus has the coreference annotation with 1560 coreference chains in 300 documents. Special multi-label model based on a language model and the set of features is developed, appropriate for presented corpus labeling. The influence of the choice of different modifications of the models: word vector representations, types of language models pre-trained for Russian, text normalization styles, and other preliminary processing are analyzed. The sufficient size of our corpus allows to study the effects of particularities of corpus labeling and balancing entities in the corpus. As a result, the state of the art for the pharmacological entity extraction problem for Russian is established on a full-size labeled corpus. In case of the adverse drug reaction (ADR) recognition, it is 61.1 by the F1-exact metric that, as our analysis shows, is on par with the accuracy level for other language corpora with similar characteristics and the ADR representativnes. The evaluated baseline precision of coreference relation extraction on the corpus is 71, that is higher the results reached on other Russian corpora.

==> tables/adr_saturation_backup2.tex <==
% \setlength{\extrarowheight}{5pt}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|} 
\hline
\diagbox{\textbf{Parameter}}{\textbf{Corpora}}                                                         &  \textbf{CADEC} & \textbf{TA} & \textbf{TT} & \textbf{TP} & \textbf{N2C2} & \textbf{PSYTAR} & \textbf{RuDRec}  \\ 
\hline
\textbf{total ADR}                                                       & 6318           & 1122        & 899         & 475         & 1579          & 4813            & 720     \\ 
\hline
\textbf{multiword (\%)}                                                 & 72.4           & 0.47        & 40          & 46.7        & 42            & 77              & 54      \\ 
\hline
\textbf{singleword (\%)}                                              & 27.6           & 0.53        & 60          & 53.3        & 58            & 23              & 46      \\ 
\hline
\textbf{discontinuous, non-overlapping (\%)}                              & 1.3            & 0           & 0           & 0           & 0             & 6.3             & 0       \\ 
\hline
\textbf{continuous, non-overlapping (\%)}                                    & 84             & 100         & 98          & 96.8        & 95            & 91.8            & 100     \\ 
\hline
\textbf{discontinuous, overlapping (\%)}                                   & 9.3            & 0           & 0           & 0           & 0             & 0.1             & 0       \\ 
\hline
\textbf{continuous, overlapping (\%)}                                        & 5.3            & 0           & 2           & 3.2         & 5             & 1.8             & 0       \\ 
\hline
\textbf{$saturation = \frac{Total\ ADR}{number\ of\ words\ in\ corpus}$ $(*10^{3})$}
         &53.38
       &NA & NA 
       &16.5 &1.35       &45.69 &10.61
       \\
\hline
$\frac{Total\ ADR} {Total\ entities\ number}$                             & 0.69           & 0.72        & 0.67        & 0.47        & 0.02          & 0.64            & 0.41    \\ 
\hline
\textbf{$\frac{Total\ ADR}{Number\ of\ Indication,\ Reason,\ etc.}$}          & 22.97          & 7.1         & 1.91          & 0.49           & 0.25          & 2.3             & 0.51       \\ 
\hline
\textbf{Estimation}                                                        & 70.6          & 61.1       & 64.8       & 73.6       & 55.8         & 71.1           & 60.4~\cite{10.1093/bioinformatics/btaa675}   \\ 
\hline
\textbf{Metric of Estimation}                                          & f1-e           & f1-am       & f1-am       & ?           & f1-r          & f1-e           & f1-e    \\
\hline
\end{tabular}

==> tables/adr_saturation_bak.tex <==
% \setlength{\extrarowheight}{5pt}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|} 
\hline
\textbf{Corpora}                                                         & \textbf{RDRS} & \textbf{CADEC} & \textbf{TA} & \textbf{TT} & \textbf{TP} & \textbf{N2C2} & \textbf{PSYTAR} & \textbf{RuDRec}  \\ 
\hline
\textbf{Total ADR}                                              & 1784          & 6318           & 1122        & 899         & 475         & 1579          & 4813            & 720     \\ 
\hline
\textbf{multiword (\%)}                                         & 64            & 72.4           & 0.47        & 40          & 46.7        & 42            & 77              & 54      \\ 
\hline
\textbf{singleword (\%)}                                        & 36            & 27.6           & 0.53        & 60          & 53.3        & 58            & 23              & 46      \\ 
\hline
\textbf{discontinuous, non-overlap (\%)}                        & 3             & 1.3            & 0           & 0           & 0           & 0             & 6.3             & 0       \\ 
\hline
\textbf{continuous, nonoverlap (\%)}                            & 80.7          & 84             & 100         & 98          & 96.8        & 95            & 91.8            & 100     \\ 
\hline
\textbf{discontinuous, overlap (\%)}                            & 0.6           & 9.3            & 0           & 0           & 0           & 0             & 0,1             & 0       \\ 
\hline
\textbf{continuous, overlap (\%)}                               & 15.8          & 5.3            & 0           & 2           & 3.2         & 5             & 1.8             & 0       \\ 
\hline
\textbf{saturation}
       &0.00425   &0.05338
       &- &- 
       &- &0.00135       &0.04569 &0.01061
       \\
\hline
$\frac{Total\ ADR} {Total\ entities\ number}$                      & 0.03          & 0.69           & 0.72        & 0.67        & 0.47        & 0.02          & 0.64            & 0.41    \\ 
\hline
\textbf{$\frac{Total\ ADR}{Number\ of\ Indication,\ Reason,\ etc.}$} & 0,38          & 22.97          & 7.1         & -           & -           & 0.25          & 2.3             & -       \\ 
\hline
\textbf{Estimation (*100\%)}                                             & –             & 70.6          & 61.1       & 64.8       & 73.6       & 55.8         & 71.1           & 60.4   \\ 
\hline
\textbf{Metric of Estimation}                                   & f1-e          & f1-e           & f1-am       & f1-am       & ?           & f1-r          & f1-e           & f1-e    \\
\hline
\end{tabular}

==> tables/cl_corp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|p{0.15\textwidth}|c|c|c|c|c|p{0.12\textwidth}|c|c|}
\hline
\multirow{2}{*}{Corpus}                            & \multicolumn{5}{c|}{Normalization}   & \multirow{2}{*}{Num. Entities} & \multirow{2}{*}{F1(exact)} & \multirow{2}{*}{F1(partial)} \\ \cline{2-6}
                                                   & SNOMED CT & MedRA & UMLS & SRD & ATC &                                &                            &                              \\ \hline
ADE corpus~\cite{li2017neural}                     & --        & +     & --   & --  & +   & 10\,666                          & 0.846                      & --                           \\ \hline
CLEF corpus~\cite{roberts2008combining}            & --        & --    & +    & --  & --  & 2\,124                           & 0.71                       & --                           \\ \hline
ShARe Clef eHealth 2013~\cite{tang2013recognizing} & +         & --    & +    & --  & --  & 11\,151                          & 0.75                       & 0.873                        \\ \hline
ShARe Clef eHealth 2014~\cite{johri2014optimizing} & +         & --    & --   & --  & --  & 19\,557                          & 0.676                      & 0.72                         \\ \hline
SCCH~\cite{shelmanov2015information}               & --        & --    & +    & +   & --  & 7\,600                           & --                         & 0.862                        \\ \hline
MADE1.0~\cite{wunnava2018bidirectional}            & --        & --    & --   & --  & --  & 79\,003                          & 0.841                      & --                           \\ \hline
I2b2 -- NLP Data Set \#3~\cite{patrick2010high} & --        & --    & --   & --  & --  & 22\,000 & 0.856                      & 0.849                           \\ \hline
IXAMed corpus~\cite{perez2017semi}                 & +         & --    & --   & --  & --  & 6\,158                           & 0.703                      & --                           \\ \hline
\end{tabular}



==> tables/clinical_corpora.tex <==
\begin{tabular}{{|p{0.1\textwidth}|p{0.325\textwidth}|p{0.15\textwidth}|p{0.325\textwidth}|}}
\hline
Corpus name             & Origin                                                                                                                                                                                           & Size                                                                                                    & Entities                                                                                                                                                                    \\ \hline
CLEF corpus             & English reports from 565\,000 records of 20\,234 deceased patients from the Royal Marsden Hospital                                                                                                 & $\sim$200 documents, 50 of each of the following types: clinical narratives, histopathology reports, and imaging reports & Condition; Drug or device; Intervention; Investigation; Laterality; Locus; Negation; Result; Sub-location
\\ \hline
ShARe Clef eHealth 2013 & English clinical reports from US intensive care (version 2.5 of the MIMIC II database). The corpus consists of discharge summaries and electrocardiogram, echocardiogram, and radiology reports & 298 documents                                                                                           & \multirow{2}{0.325\textwidth}{
    Negation Indicator; Subject Class; Uncertainty Indicator; Course Class; Severity Class; Conditional Class; Generic Class; Body Location; DocTime Class; Temporal Expression}
\\ \hline
ShARe Clef eHealth 2014 & English clinical reports (same as CLEF 2013)                                                                                                                                                  & 433 documents                                                                                           & Negation Indicator; Subject Class; Uncertainty Indicator; Course Class; Severity Class; Conditional Class; Generic Class; Body Location; DocTime Class; Temporal Expression
\\ \hline
SCCH                    & Russian clinical records for 60 patients from Federal State Autonomous institution ``National Medical Research Center of Children Health'' (NMRCCH)                                                & 112 documents                                                                                           & Disease; Symptom; Drug; Treatment; Body location; Severity; Course
\\ \hline
ADE corpus              & English medical case reports of MEDLINE database, which is a part of PubMed. The documents with medication adverse effects mentioned are selected.                                                 & 2\,972 documents                                                                                         & Drug; Adverse effect; Dosage
\\ \hline
MADE1.0                 & English medical records of 21 randomly selected cancer patients monitored in the University of Massachusetts Memorial Hospital                                                                       & 1\,089 notes                                                                                             & Adverse effect; Indication; Other Sign, Symptom, or Disease; Severity; Drugname; Dosage; Duration; Frequency; Route
\\ \hline
I2b2 – NLP Data Set \#3  & English discharge summaries of patients from the non-profit hospital and physicians network ``Partners Healthcare''                     & 1\,243 documents                                                                                         & Medications; Dosages; Modes; Frequencies; Durations; Reasons; List/narrative
\\ \hline
IxaMed corpus           & Randomly selected reports of Spanish medical consultations in Galdakao-Usansolo Hospital                                                                                                         & 75 verified reports                                                                                     & Drug; Procedure; Disease
\\ \hline
\end{tabular}


==> tables/compare_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{tabular}{|c|c|c|c|}
\hline
                                                                                             & Method                                                                        & $\Fp$ & $\Fe$    \\ \hline
\multicolumn{4}{|c|}{\cellcolor[HTML]{C0C0C0}ADR}                                                                                                                                                               \\ \hline
Our model                                                                                    & \begin{tabular}[c]{@{}c@{}}ELMo, BERT, CRF, pos, \\ 3-layer LSTM\end{tabular} & 68.8 $\pm$ 1.5 & 78.84 $\pm$ 2.8
\\ \hline
                                                                                             & 3-layer GRU, CNN, CRF                                                         & 70.65          & 79.78           \\ \cline{2-4} 
\multirow{-2}{3cm}{Tutubalina E. et al., 2017~\cite{tutubalina2017combination}}        & 3-layer LSTM, CNN, CRF                                                        & 69.65          & 81.15           \\ \hline
\multicolumn{4}{|c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} Disease + Drug}}                                                                                                                             \\ \hline
Our model                                                                                    & \begin{tabular}[c]{@{}c@{}}ELMo, BERT, CRF, pos, \\ 3-layer LSTM\end{tabular} & 75.6 $\pm$ 1.4 & 86.3 $\pm$ 0.7  \\ \hline
                                                                                             & \begin{tabular}[c]{@{}c@{}}CRF,\\ HealthVec, all features\end{tabular}        & 69.1           & 79.4            \\ \cline{2-4} 
\multirow{-2}{3cm}{Miftahutdinov Z. Sh. et al., 2017~\cite{miftahutdinov2017identifying}} & 3-layer LSTM, HealthVec                                                       & 67             & 81.2            \\ \hline
\end{tabular}


==> tables/compare_dialog.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{}                                                                                                             & \multicolumn{2}{c|}{\multirow{2}{*}{Method}}                                                      & \multicolumn{2}{c|}{Disease + Drug} \\ \cline{4-5} 
                                                                                                                              & \multicolumn{2}{c|}{}                                      & $f1_{partial}$    & $f1_{exact}$    \\ \hline
Our model                                                                                                                     & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}ELMO,\\ BERT, CRF, pos, 3-layer LSTM\end{tabular}} & 75.6 $\pm$ 1.4      & 86.3 $\pm$ 0.7    \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Miftahutdinov Z. Sh. et al.\\ \cite{miftahutdinov2017identifying},2017\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}CRF,\\ HealthVec, all features\end{tabular}}       & 69.1              & 79.4            \\ \cline{2-5} 
                                                                                                                              & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}3-layer\\ LSTM,  HealthVec\end{tabular}}           & 67                & 81.2            \\ \hline
\end{tabular}


==> tables/compare_hindawi.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{}                                                                                                   & \multicolumn{2}{c|}{\multirow{2}{*}{Method}}                                                      & \multicolumn{2}{c|}{ADR}        \\ \cline{4-5} 
                                                                                                                    & \multicolumn{2}{c|}{}                                      & $f1_{partial}$ & $f1_{exact}$   \\ \hline
Our model                                                                                                           & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}ELMO,\\ BERT, CRF, pos, 3-layer LSTM\end{tabular}} & 68.8 $\pm$ 1.5   & 78.84 $\pm$ 2.8  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Tutubalina E. et al.\\ \cite{tutubalina2017combination},2017\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}3-layer\\ GRU + CNN + CRF\end{tabular}}            & \textbf{70.65} & 79.78          \\ \cline{2-5} 
                                                                                                                    & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}3-layer\\ LSTM + CNN + CRF\end{tabular}}           & 69.65          & \textbf{81.15} \\ \hline
\end{tabular}



==> tables/general_inf_about_corpus.tex <==
% \usepackage{multirow}
\begin{tabular}{|l|l|l|p{0.095\textwidth}|p{0.07\textwidth}|l|l|l|l|} 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Entity type \end{tabular}} & \multicolumn{4}{c|}{Entities}                              & \multicolumn{2}{l|}{MEHSRUS} & \multicolumn{2}{l|}{MEHSRUS-2}  \\ 
\cline{2-9}
                                                                                   & Annotated   & Standardized & Num. words relating to entities & Reviews coverage & total & unique               & total & unique                  \\ 
% \cline{1-1}
\hline
ADR                                                                                & 844    & 163    & 4 159                            & 448              & 455   & 112                  & 0     & 0                       \\ 
\hline
Medication                                                                         & 17 779 & 1 719   & 52 782                          & 1 659             & 3 612  & 458                  & 1 234  & 131                     \\ 
\hline
Drugname                                                                           & 4 730  & 384    & 7 497                            & 1 654             & 852   & 166                  & 47    & 14                      \\ 
\hline
DrugBrand                                                                          & 2 564  & 235    & 2 936                           & 1 036             & 23    & 19                   & 2     & 1                       \\ 
\hline
Drugform                                                                           & 3 236  & 31     & 6 496                            & 1 243             & 651   & 40                   & 368   & 48                      \\ 
\hline
Drugclass                                                                          & 1 735  & 43     & 4 069                            & 974              & 682   & 47                   & 624   & 35                      \\ 
\hline
MedMaker                                                                           & 998    & 210    & 2 838                            & 851              & 553   & 60                   & 178   & 25                      \\ 
\hline
Frequency                                                                          & 365    & 122    & 2 805                            & 303              & 6     & 5                    & 0     & 0                       \\ 
\hline
Dosage                                                                             & 506    & 95     & 2 632                            & 387              & 20    & 9                    & 1     & 1                       \\ 
\hline
Duration                                                                           & 897    & 86     & 4 012                            & 703              & 9     & 9                    & 0     & 0                       \\ 
\hline
Route                                                                              & 1 511  & 504    & 6 646                            & 834              & 288   & 65                   & 14    & 7                       \\ 
\hline
SourceInfodrug                                                                     & 1 225  & 9      & 4 733                           & 861              & 528   & 38                   & 0     & 0                       \\ 
\hline
Disease                                                                            & 9 285  & 4 462   & 39 548                           & 1 603             & 3 272  & 791                  & 82    & 16                      \\ 
\hline
Diseasename                                                                        & 2 235  & 141    & 5 059                            & 921              & 499   & 55                   & 76    & 12                      \\ 
\hline
Indication                                                                         & 2 334  & 708    & 7 230                           & 971              & 757   & 112                  & 3     & 1                       \\ 
\hline
BNE-Pos                                                                            & 2 967  & 1 301   & 15 932                           & 1 021             & 794   & 185                  & 1     & 1                       \\ 
\hline
ADE-Neg                                                                            & 115    & 94     & 906                            & 68               & 58    & 43                   & 0     & 0                       \\ 
\hline
NegatedADE                                                                         & 1 535  & 604    & 9 617                            & 641              & 260   & 97                   & 2     & 2                       \\ 
\hline
Worse                                                                              & 83     & 68     & 696                            & 51               & 29    & 21                   & 0     & 0                       \\ 
\hline
Note                                                                               & 2 319  & 1 546   & 19 781                           & 1 004             & 875   & 278                  & 2     & 2                       \\
\hline
\end{tabular}


==> tables/general_inf_about_corpus_2_backupWithMesh.tex <==
% \usepackage{multirow}
\begin{tabular}{|l|l|p{0.13\textwidth}|p{0.12\textwidth}|p{0.075\textwidth}|p{0.07\textwidth}|l|l|l|l|} 
\hline
\multirow{2}{*}{Entity type} & \multicolumn{4}{c|}{Mentions}                              & \multicolumn{2}{c|}{MESHRUS} & \multicolumn{2}{c|}{MESHRUS-2}  \\ 
\cline{2-9}
                                                                                   & Annotated   & Classification \& normalization & Num. words in the mentions & Reviews coverage & total & unique               & total & unique                  \\ 
% \cline{1-1}
\hline
ADR & 1784 & 316 (MedDRA) & 4 211 & 628 & 455   & 112                  & 0     & 0                       \\ 
\hline
Medication                                                                         & 32 994 &    & 47 306 & 2 799             & 3 612  & 458                  & 1 234  & 131                     \\ 
\hline
Drugname                                                                           & 8 236  & 550(SRD), 226(ATC)    & 9 914                         & 2 793 & 852   & 166                  & 47    & 14                      \\ 
\hline
DrugBrand                                                                          & 4 653  &     & 5 296                        & 1 804             & 23    & 19                   & 2     & 1                       \\ 
\hline
Drugform & 5 994  &  & 6 131 & 2 193             & 651   & 40                   & 368   & 48                      \\ 
\hline
%Drugclass                                                                          & 1 735  & 42     & 4 069 & 1 204                           & 974              & 682   & 47                   & 624   & 35                      \\
Drugclass & 3 120  & 70 (ATC) & 3 277 & 1 687              & 682   & 47                   & 624   & 35                      \\ 
\hline
MedMaker                                                                           & 1 715    &     & 2 423 & 1 448              & 553   & 60                   & 178   & 25                      \\ 
\hline
Frequency                                                                          & 614    &     & 2 478 & 516              & 6     & 5                    & 0     & 0                       \\ 
\hline
Dosage                                                                             & 965    &      & 2 389 & 708              & 20    & 9                    & 1     & 1                       \\ 
\hline
Duration                                                                           & 1 514    &      & 3 137 & 1 194              & 9     & 9                    & 0     & 0                       \\ 
\hline
Route                                                                              & 3 617  &     & 7 869                           & 1 737              & 288   & 65                   & 14    & 7                       \\ 
\hline
SourceInfodrug                                                                     & 2 566  &       & 4 392 & 1 579              & 528   & 38                   & 0     & 0                       \\ 
\hline
Disease                                                                            & 17 332  &    & 37 863 & 2 712             & 3 272  & 791                  & 82    & 16                      \\ 
\hline
Diseasename                                                                        & 4 006  & 247 (ICD-10)    & 4 713 & 1 621              & 499   & 55                   & 76    & 12                      \\ 
\hline
Indication & 4 606  & 343 (MedDRA) & 7 858 & 1 784              & 757   & 112                  & 3     & 1                       \\ 
\hline
BNE-Pos                                                                            & 5 613  &    & 14 883 & 1 764             & 794   & 185                  & 1     & 1                       \\ 
\hline
ADE-Neg                                                                            & 85    &      & 347 & 54               & 58    & 43                   & 0     & 0                       \\ 
\hline
NegatedADE                                                                         & 2 798  &     & 9 028 & 1 104              & 260   & 97                   & 2     & 2                       \\ 
\hline
Worse                                                                              & 224     &      & 1 034 & 134               & 29    & 21                   & 0     & 0                       \\ 
\hline
Note                                                                               & 4 517  &    & 21 200 & 1 876             & 875   & 278                  & 2     & 2                       \\
\hline
\end{tabular}


==> tables/meshrus_stat.tex <==
% \usepackage{multirow}
\begin{tabular}{|l|l|l|l|l|} 
\hline
\multirow{2}{*}{Entity type} &   \multicolumn{2}{c|}{MESHRUS} & \multicolumn{2}{c|}{MESHRUS-2}  \\ 
\cline{2-5}
    &  total & unique  & total & unique    \\ 
% \cline{1-1}
\hline
ADR & 455   & 112 & 0 & 0   \\ 
\hline
Medication   &  3 612  & 458  & 1 234  & 131  \\ 
\hline
Drugname & 852   & 166   & 47    & 14 \\ 
\hline
DrugBrand  & 23    & 19 & 2     & 1  \\ 
\hline
Drugform  & 651   & 40   & 368   & 48 \\ 
\hline
Drugclass &  682   & 47  & 624   & 35 \\ 
\hline
MedMaker & 553   & 60  & 178   & 25  \\ 
\hline
Frequency  & 6     & 5  & 0     & 0   \\ 
\hline
Dosage  & 20    & 9   & 1     & 1    \\ 
\hline
Duration  & 9     & 9    & 0     & 0     \\ 
\hline
Route  & 288   & 65   & 14    & 7    \\ 
\hline
SourceInfodrug  & 528   & 38    & 0     & 0   \\ 
\hline
Disease  & 3 272  & 791  & 82    & 16   \\ 
\hline
Diseasename  & 499   & 55  & 76    & 12     \\ 
\hline
Indication & 757   & 112   & 3     & 1     \\ 
\hline
BNE-Pos  & 794   & 185  & 1     & 1     \\ 
\hline
ADE-Neg   & 58    & 43       & 0     & 0         \\ 
\hline
NegatedADE  & 260   & 97    & 2     & 2   \\ 
\hline
Worse  & 29    & 21                   & 0     & 0                       \\ 
\hline
Note  & 875   & 278                  & 2     & 2                       \\
\hline
\end{tabular}


==> tables/open_access_subsets.tex <==
\setlength\tabcolsep{2.2pt}
\begin{tabular}{|p{90pt}|c|c|c|} 
\hline
\diagbox{\textbf{Params}}{\textbf{Corpora}}                                & \textbf{RuDRec}  & \textbf{CADEC} & \textbf{RuDRec}   \\ 
\hline
\textbf{Number of reviews }                      & 500                             & 1250           & 500                              \\ 
\hline
\textbf{Number of reviews contained ADR }        & 203                             & 1107           & 203                              \\ 
\hline
\textbf{Portion of reviews contained ADR }       & 0.41                            & 0.89           & 0.41                             \\ 
\hline
\textbf{Number of ADR entitites }                & 720                             & 6318           & 720                              \\ 
\hline
\textbf{Average number of ADR per review }       & 1.4                             & 5.05           & 1.4                              \\ 
\hline
\textbf{Number of reviews contained Indication } & 500                             & 168            & 500                              \\ 
\hline
\textbf{Total entitites number }                 & 4565                            & 9111           & 4565                             \\ 
\hline
\textbf{Number of Indication entitites }         & 1401                            & 275            & 1401                             \\ 
\hline
\textbf{Portion of ADR to Indication entities }  & 0.51                            & 22.97          & 0.51                             \\ 
\hline
\textbf{F1-exact }                               & $62.73 \pm 3.41$ & 70.60          & $60.36 \pm 2.13$  \\ 
\hline
\textbf{Saturation}                              & 0.010608                               & 0.053381293              & 0.010608                                \\
\hline
\end{tabular}

==> tables/rdrs_subsets_backup <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|c|}
\hline
\textbf{Corpora} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Number \\ of \\ reviews\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Number \\ of reviews \\ contained \\ ADR\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Portion of \\ reviews \\ contained \\ ADR\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Number of \\ ADR \\ entitites\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}} Average \\ number \\ of ADR \\ per \\ Review\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Number of \\ reviews \\ contained \\ Indication\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Total \\ entitites\\ number\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Number of \\ Indication \\ entitites\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Portion of \\ ADR to \\ Indication \\ entities\end{tabular}}} & \textbf{F1-exact}                                       \\ \hline
RDRS\_2800 & 2800  & 625  & 0.22  & 1778 & 0.64 & 1783  & 52186  & 4627 & 0.38  & 52.784 \pm 3.756 \\ \hline
RDRS\_1660 & 1659 & 339 & 0.2 & 843 & 0.51 & 955 & 27987 & 2310 & 0.36 & 40.1\pm2.9 \\ \hline
\begin{tabular}[c]{@{}l@{}}RDRS\_1250 \\ (balanced)\end{tabular} & 1250 & 610 & 0.49 & 1752 & 1.4 & 670 & 21807 & 1518 & 1.15 & 61.12\pm1.514  \\ \hline
RDRS\_610 & 610 & 610  & 1 & 1750 & 2.9 & 59 & 3782 & 90 & 19.44 & 71.282\pm3.388 \\ \hline
RDRS\_1136 & 1136 & 610 & 0.54 & 1750 & 1.54  & 154  & 6126 & 237 & 7.38 & 68.564\pm3.27 \\ \hline
RDRS\_500 & 500 & 177 & 0.35 & 709 & 1.4 & 297  & 9495 & 720 & 0.98 & \multicolumn{1}{l|}{надо досчитать}                     \\ \hline
\begin{tabular}[c]{@{}l@{}}RuDRec\\ (labeled part)\end{tabular}  & 500  & 203 & 0.41 & 720 & 1.4 & 500 & 4565 & 1401 & 0.51 & 62.732\pm3.405 \\ \hline
\multicolumn{11}{|c|}{\textbf{Open access data}} \\ \hline
CADEC & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{}  & 6318 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{0,706~\cite{li2020lexicon}}   \\ \hline
\begin{tabular}[c]{@{}l@{}}RuDRec \\ (labeled part)\end{tabular} & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{}  & 720 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{0.604~\cite{tutubalina2020russian}} \\ \hline
\end{tabular}


==> tables/relevant_corpus.tex <==
\begin{tabular}
{|p{0.2\textwidth}|p{0.2\textwidth}|p{0.2\textwidth}|p{0.25\textwidth}|}
\\ \hline

\textbf{Corpus name}                                                 & \textbf{Origin}                                                                                                                                                                                  & \textbf{Size}                                                                                                                              & \textbf{Entities}                                                                                                                                                           \\ \hline
\endhead
\hline \multicolumn{4}{|r|}{{Continued on next page}} \\ \hline
\endfoot


CLEF corpus \cite{roberts2007clef}                  & English reports from the 565k records of 20234 deceased patients from the Royal Marsden Hospital                                                                                                 & $\sim$200 documents. 50 of each type: clinical narratives, histopathology reports, and imaging reports, and another unclear described part & Condition; Drug or device; Intervention; Investigation; Laterality; Locus; Negation; Result; Sub-location                                                                   \\ \hline
ShARe Clef eHealth 2013 \cite{pradhan2013task}      & English clinical reports from US intensive care (version 2.5 of the MIMIC II database). The corpus consisted of discharge summaries and electrocardiogram, echocardiogram, and radiology reports & 298 documents                                                                                                                              & Negation Indicator; Subject Class; Uncertainty Indicator; Course Class; Severity Class; Conditional Class; Generic Class; Body Location; DocTime Class; Temporal Expression \\ \hline
ShARe Clef eHealth 2014 \cite{mowery2014task}       & English clinical reports (same as at CLEF 2013)                                                                                                                                                  & 433 documents                                                                                                                              & Negation Indicator; Subject Class; Uncertainty Indicator; Course Class; Severity Class; Conditional Class; Generic Class; Body Location; DocTime Class; Temporal Expression \\ \hline
SCCH \cite{shelmanov2015information}                & Russian clinical records for 60 patients from  Federal State Autonomous institution ''National Medical Research Center of Children Health'' (NMRCCH)                                               & 112 documents                                                                                                                              & Disease; Symptom; Drug; Treatment; Body location; Severity; Course                                                                                                          \\ \hline
ADE corpus \cite{gurulingappa2012development}       & English medical case reports of MEDLINE database, that is part of PubMed. The documents with mentioned medications adverse effects are selected.                                                    & 2972 documents                                                                                                                            & Drug; Adverse effect; Dosage                                                                                                                                                \\ \hline
MADE1.0 \cite{jagannatha2019overview}               & English medical records of 21 randomly selected cancer patients monitored in University of Massachusetts Memorial Hospital                                                                       & 1089 notes                                                                                                                                & Adverse effect; Indication; Other Sign, Symptom, or Disease; Severity; Drugname; Dosage; Duration; Frequency; Route                                                         \\ \hline
I2b2 -- NLP Data Set \#3 \cite{uzuner2010extracting} & English discharge summaries of patients from the non-profit hospital and physicians network ''Partners Healthcare''                                                                                & 1243 documents                                                                                                                            & Medications; Dosages; Modes; Frequencies; Durations; Reasons; List/narrative                                                                                                \\ \hline
IxaMed corpus \cite{oronoz2015creation}             & Randomly selected reports of Spanish medical consultations in Galdakao-Usansolo Hospital                                                                                                         & 75 verified reports                                                                                                                        & Drug; Procedure; Disease                                                                                                                                                    \\ \hline

\end{tabular}

==> tables/result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{}                                                                                    & \multicolumn{2}{c|}{ADR}      & \multicolumn{2}{c|}{Medication} & \multicolumn{2}{c|}{Disease}  \\ \cline{2-7} 
                                                                                                     & $f1_{partial}$ & $f1_{exact}$ & $f1_{partial}$  & $f1_{exact}$  & $f1_{partial}$ & $f1_{exact}$ \\ \hline
\begin{tabular}[c]{@{}c@{}}ELMO, ton, pos,\\  UMLS, UMLS2, Vidal, CRF, \\ 3-layers LSTM\end{tabular} & 48.7 \pm 5.6   & 32.4 \pm 4.7 & 86.5 \pm 0.6    & 74.6 \pm 1.1  & 73.2 \pm 0.7   & 52.3 \pm 1.4 \\ \hline
\begin{tabular}[c]{@{}c@{}}ELMO, BERT, ton,\\ 3-layers LSTM\end{tabular}                             & -              & -            & 86.1 \pm 0.7    & 75.6 \pm 0.4  & -              & -            \\ \hline
\end{tabular}
\end{table}


==> tables/social_corpora.tex <==
\begin{tabular}{|p{0.25\textwidth}|p{0.25\textwidth}|p{0.25\textwidth}|p{0.25\textwidth}|} 
\\ \hline
\textbf{Corpus name}                                                 & \textbf{Origin}                                                                                                                                                                                  & \textbf{Size}                                                                                                                              & \textbf{Entities}                                                                                                                                                           \\ \hline
CADEC \cite{karimi2015cadec}                        & English user reviews on drugs (12 medication names) from the "AskaPatient" medical forum
& 1253 posts
& Drug; Adverse effect; Disease; Symptom; Finding 
\\ \hline

TwiMed corpus \cite{alvaro2017twimed}               & English twitter posts and sentences from Pubmed texts contained                                                                                                                                  & 1000 tweets and 1000  sentences                                                                                                           & Drug; Disease; Symptom                                                                                                                                                      \\ \hline
Twitter annotated corpus \cite{sarker2016social}    & English twitter posts containing ADR mentions (Pre-selected by the presence of generic or brand drug names in dictionaries)                                                                          & 110\,833 tweets with binary labels for ADR (1239 contain ADR), 1783 texts have entities markup                                             & Adverse drug reaction; Beneficial effect; Indication; Other                                                                                                                 \\ \hline
PsyTar dataset \cite{zolnoori2019psytar}            & English forum messages about psychiatric drugs effects from the askapatient.com website                                                                                                                 & 891 reviews (6004 sentences)                                                                                                               & Adverse drug reaction; Withdrawal Symptoms; Sign, Symptom, Illness; Drug Indications; Drug Effectiveness; Drug Ineffectiveness                                              \\ \hline
\end{tabular}

==> tables/table3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
%\usepackage{multirow}
\begin{tabular}{|p{0.1\linewidth}|c|c|c|c|c|p{0.12\linewidth}|c|c|}
\hline
\multirow{2}{*}{Corpus}                         & \multicolumn{5}{c|}{Assignment of entities to the thesaurus }     & \multirow{2}{*}{Num. Entities}             & \multirow{2}{*}{F1(exact)} & \multicolumn{1}{l|}{\multirow{2}{*}{F1(partial)}} \\ \cline{2-6}
                                                & SNOMED CT & MedRA & UMLS & SIDER & AMT &                                            &                            & \multicolumn{1}{l|}{}                             \\ \hline
CADEC~\cite{dai2017medication}                  & +         & +     & --   & --    & +   & 8118                                       & 0.806                      & --                                                \\ \hline
PsyTar~\cite{zolnoori2019systematic}            & +         & --    & +    & --    & --  & 7414                                       & 0.64~\cite{basaldella2019bioreddit}                      & --                                                \\ \hline
TwiMed~\cite{gupta2018multi}                    & +         & +     & --   & +     & --  & 1200                                       & --                         & 0.648                                             \\ \hline
Twitter annotated corpus~\cite{wang2016mining} & --        & --    & +    & --    & --  & 1482 tweets (2130 tweets original dataset) & --                         & 0.611                                             \\ \hline
\end{tabular}

==> tables/table4.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{tabular}{|p{0.18\textwidth}|p{0.17\textwidth}|p{0.18\textwidth}|p{0.17\textwidth}|p{0.17\textwidth}|}
% \hline
% Paper               & Text type                           & Corpus                & Number of ADR entities & F1 (exact) \\ \hline
% Li Z. et. al.~\cite{li2020lexicon}   & \multirow{3}{*}{Social media}       & Cadec                 & 6318                   & 0.706      \\ \cline{1-1} \cline{3-5} 
% Gupta et. al.~\cite{gupta2018multi}       &                                     & TwiMed (Twitter part) & $\sim$1200             & 0.648       \\ \cline{1-1} \cline{3-5} 
% W. Wang~\cite{wang2016mining}             &                                     & Twitter annotated corpus              &           NA             & 0.611       \\ \hline
% Ramamoorthy et. al.~\cite{li2017neural} & \multirow{2}{*}{Clinical documents} & ADE corpus                  & 5776                   & 0.868       \\ \cline{1-1} \cline{3-5} 
% Wunnava et. al.~\cite{wunnava2018bidirectional}     &                                     & MADE1.0                  & 1940                   & 0.609       \\ \hline
% \end{tabular}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Text type}                           & \textbf{Paper}                                  & \textbf{Corpus}          & \textbf{Number of ADR entities} & \textbf{F1 (exact)} \\ \hline
\multirow{3}{*}{Social media}       & Li Z. et. al.~\cite{li2020lexicon}              & Cadec                    & 6318                            & 0.706               \\ \cline{2-5} 
                                    & Gupta et. al.~\cite{gupta2018multi}             & TwiMed (Twitter part)    & $\sim$1200                      & 0.648               \\ \cline{2-5} 
                                    & W. Wang~\cite{wang2016mining}                   & Twitter annotated corpus & NA                              & 0.611               \\ \hline
\multirow{2}{*}{Clinical documents} & Ramamoorthy et. al.~\cite{li2017neural}         & ADE corpus               & 5776                            & 0.868               \\ \cline{2-5} 
                                    & Wunnava et. al.~\cite{wunnava2018bidirectional} & MADE1.0                  & 1940                            & 0.609               \\ \hline
\end{tabular}


==> tables/table6.tex <==
\begin{tabular}{|p{0.1\textwidth}|p{0.2\textwidth}|p{0.1\textwidth}|p{0.1\textwidth}|p{0.38\textwidth}|}
\hline
\multicolumn{1}{|c|}{Type} & \multicolumn{1}{c|}{Origin}            & \multicolumn{1}{c|}{Size} & \multicolumn{1}{c|}{Language} & \multicolumn{1}{c|}{Named Entities}                                          

\\ \hline
Social                              & Reviews from users of the Otzovik medical forum & 2800 posts                         & Russian                                & ADR; Medication (Drugname; DrugBrand; Drugform; Drugclass; Domestic; Foreign; Frequency; Dosage; Duration; Route; SourceInfodrug); Disease (Diseasename; Indication; ADE-Neg; BNE-Pos; NegatedADE; Notes; Worse); Note \\ \hline
\end{tabular}

==> tables/table_drugs_stat.tex <==
\begin{tabular}{|p{0.133\textwidth}|p{0.133\textwidth}|p{0.133\textwidth}|}
\hline
                      & Number of a unique drugs & Drugs entries number \\ \hline
Reviewed in more then 20 docs & 29                                & 1 114 (47.2\%)                 \\ \hline
Top 20\%     & 77                                & 1 699 (71.99\%)                \\ \hline
Total        & 384                               & 2 360 (100\%)                  \\ \hline
\end{tabular}


==> tables/table_undesirable_reactions_stat.tex <==
\begin{tabular}{|p{0.133\textwidth}|p{0.133\textwidth}|p{0.133\textwidth}|}
\hline
                   & ADR number & Different ADR entries number \\ \hline
ADR Top-20 & 20                                          & 466 (62.88\%)                                           \\ \hline
Total     & 163                                         & 741 (100\%)                                             \\ \hline
\end{tabular}
